Cleanformer: A multichannel array configuration-invariant neural enhancement frontend for ASR in smart speakers

This work introduces the Cleanformer, a streaming multichannel neural based enhancement frontend for automatic speech recognition (ASR). This model has a conformer-based architecture which takes as inputs a single channel each of raw and enhanced signals, and uses self-attention to derive a time-frequency mask. The enhanced input is generated by a multichannel adaptive noise cancellation algorithm known as Speech Cleaner, which makes use of noise context to derive its filter taps. The time-frequency mask is applied to the noisy input to produce enhanced output features for ASR. Detailed evaluations are presented with simulated and re-recorded datasets in speech-based and non-speech-based noise that show significant reduction in word error rate (WER) when using a large-scale state-of-the-art ASR model. It also will be shown to significantly outperform enhancement using a beamformer with ideal steering. The enhancement model is agnostic of the number of microphones and array configuration and, therefore, can be used with different microphone arrays without the need for retraining. It is demonstrated that performance improves with more microphones, up to 4, with each additional microphone providing a smaller marginal benefit. Specifically, for an SNR of -6dB, relative WER improvements of about 80\% are shown in both noise conditions.

==> 5.corrupt.tex <==


\section{``Corrupt" Noise Context}
\label{sec:corrupt_context}

Thus far, the assumption has been made that the desired speaker was not present in the noise context. In this section we shall examine the impact of the failure of this assumption to be met and present techniques for mitigating the impact.

This assumption is important due to the Speech Cleaner. The noise cancellation filter adapts during the noise context to cancel out what it encounters. During the query, adaptation has stopped and both desired speech and interfering audio are filtered. The filter attenuates the interfering audio which it encountered during adaptation while letting the desired speech that was not present during training pass through. When that desired speaker is also present during the noise context, the Speech Cleaner will work to remove that speaker as well. Although this does not happen in the majority of the use cases we encounter, it is still an important edge-case.

First we look at the performance when the desired speaker is present in the noise context. To understand the impact and to give a worst case evaluation of performance, test sets were derived where the noise contexts were replaced with the queries themselves. This ensures that the desired speaker is present throughout the noise context. Results are shown in Table \ref{tab:corrupt context} for simulated three microphone LibriSpeech sets with added environmental and speech-based noise. The first row shows the baseline. The next line shows the Speech Cleaner which will erase much of the desired speaker because it was present in the noise context. The third line shows the Cleaned Mask which lowers the impact of the Speech Cleaner due to the mask scalar still resulting in deterioration but less of it. The penultimate line shows performance with Cleanformer. Like Speech Cleaner, the impact on performance is catastrophic with almost all 100\% errors. In the four previous cases, errors are largely deletions resulting from the enhanced input having the desired speaker attenuated. 

To address this Cleanformer was retrained using a corrupt context 20\% of the time. In half of those cases the query was used as the context and in the other half white noise was used for the noise context. With white noise as the noise context, Speech Cleaner does not learn anything useful to remove noise in the query portion of the input audio. The third row in Table shows the performance of the retrained Cleanformer (Cleanformer$++$). While this does not attain the performance improvement of the Cleaner in the intended conditions, the retrained Cleanformer does not exhibit the catastrophic failures under these conditions observed with the original Cleanformer. In fact, relative to the baselines, improvements are observed with Cleanformer$++$ ranging from 11\% to 30\% relative WER improvement. This is likely because Cleanformer$++$ has learned to suppress background noise without fully relying on Speech Cleaner, and making best possible use of the available partial information.

Next, we look at the impact that training the Cleanformer with some fraction of utterances with ``corrupt" noise context has on performance under the intended conditions when the desired speaker is absent during the noise context. Table \ref{tab:retrained model} compares the re-trained Cleanformer with the original. Cleanformer$++$ shows similar performance to the original Cleanformer across the considered conditions, maintaining the significant improvement over the baseline. 

These results suggest that training the Cleanformer with some utterances having a ``corrupt" noise context enables it to tolerate the cases where the  desired speaker is present in the noise context. Under the intended conditions the Cleanformer$++$ has similar performance to the original Cleanformer. 



